Towards a General Model of Knowledge for Facial Analysis by Multi-Source Transfer Learning

This paper proposes a step toward obtaining general models of knowledge for facial analysis, by addressing the question of multi-source transfer learning. More precisely, the proposed approach consists in two successive training steps: the first one consists in applying a combination operator to define a common embedding for the multiple sources materialized by different existing trained models. The proposed operator relies on an auto-encoder, trained on a large dataset, efficient both in terms of compression ratio and transfer learning performance. In a second step we exploit a distillation approach to obtain a lightweight student model mimicking the collection of the fused existing models. This model outperforms its teacher on novel tasks, achieving results on par with state-of-the-art methods on 15 facial analysis tasks (and domains), at an affordable training cost. Moreover, this student has 75 times less parameters than the original teacher and can be applied to a variety of novel face-related tasks.

==> annexe.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llll}
\hline
Task            & Features size & Architecture  & Source               \\ \hline
ImageNetClassif & 2048          & ResNet-101    & Pytorch              \\
DiscreteEmotion & 376           & PyramidNet-50 & Ours on AffectNet    \\
FaceAttributes  & 376           & PyramidNet-50 & Ours on CelebA       \\
Age             & 512           & ResNet-50     & Antipov et al. CVPRW \\
Gender          & 128           & ResNet-50     & Antipov et al.       \\
Identity        & 2048          & ResNet-50     & Baccouche at Orange Labs  \\ \hline
\end{tabular}
\label{models}
\caption{Pretrained models of the bank}
\end{table}

\begin{table}[ht]
\begin{tabular}{lll}
\hline
Model type       & Time on $\mathcal{D}_{unsup}$ & Time on RAF \\ \hline
Extraction       & 50                            & 0.15        \\ \hline
MLP              &                               & 0.05        \\
PCA              & 7                             & 0.04        \\
AE               & 18                            & 0.04        \\ \hline
BT               &                               & 0.24        \\
BCT              &                               & 15          \\ \hline
CNN              &                               & 0.42        \\
MT-CNN           & 76                            & 0.21        \\
$\mathcal{S}$-CF &                               & 0.12        \\
$\mathcal{S}$-WF & 70                            & 0.21        \\ \hline
\end{tabular}
\caption{Training time (in hours with one GPU) for different approaches on $\mathcal{D}_{unsup}$ (when relevant) and on one evaluation dataset (RAF). }
\end{table}

==> experiments.tex <==
\section{Experiments}
This section presents an experimental validation of the proposed method. In these experiments, we want to extract information from 6 existing models trained to address 6 tasks (facial expression recognition, age regression, identity prediction, gender recognition, attribute detection, object recognition), and evaluate the transfer of this information to 10 related tasks but with different domains. 

After giving detailed information about the tasks considered and some implementation details, we successively present some ablative experiments on the Teacher model as well as on the Student model, discuss the performance of the student on the original tasks and, finally, comment on training times.

\subsection{Tasks and Datasets\label{sec:datasets}}
\paragraph{Existing (pre-trained) models}
As the existing models are seen as sources of knowledge, a main concern when choosing them is to know on which domain they were trained in order to avoid any overlaps with data used during evaluation. It is the reason why we choose to train by ourselves the 6 models following state-of-the-art approaches, instead of using some pre-existing models provided by their authors. Thus we can give the guarantee there is no overlapping data.
We explain below how the different models are trained.\\
\noindent\emph{\underline{Expr-AffectNet}: classifying a face among 7 facial expressions.}
We follow a similar approach to~\cite{vielzeuf2018occam}, but we train a PyramidNet-50~\cite{DPRN} instead of a ResNet~\cite{he2016deep} on 300,000 faces extracted from the AffectNet dataset~\cite{mollahosseini2017affectnet}. The last hidden layer of the model is of size 376. The obtained accuracy on 7 classes on the AffectNet validation set is of 63.5\% (note that the 'contempt' label was removed).\\
\emph{\underline{Identity-MS}: predicting identity by pairwise comparison}
We implement a ResNet-50 trained on a subset of MS-Celeb~\cite{guo2016ms} and apply the methods described in ~\cite{schroff2015facenet}. The last hidden layer of the model is of size 2048. We reach 99.65\% accuracy on LFW~\cite{lfw}, a dataset of 13,233 faces. We follow the unrestricted, labeled outside data protocols and therefore compute L2 distance between embedding pairs and calculate the average accuracy for each given fold. The threshold on the distance between positive and negative pairs is set as the best threshold on the other 9 folds. The average accuracy is evaluated on the 10 folds.\\
\emph{\underline{AgeR-IMDB}: regressing the age of a given face.}
We implement a ResNet-50 defined and trained exactly as in~\cite{antipov2017effective} on a subset of IMDB-WIKI using a Label Distribution Age Encoding (LDAE) loss. The last hidden layer of the model is of size 512 because the ResNet-50 final layers are modified into a Multi Layer Perceptron with two layers (2048 to 512 and 512 to 100). We were able to reproduce similar results to the original paper with a MAE of 2.85 on FG-NET.\\
\emph{\underline{Gender-IMDB}: predicting the gender of a given face.}
The identity ResNet-50 previously described was fine-tuned on the gender prediction task, modifying the last layer into a Multi Layer Perceptron with two layers (2048 to 128 and 128 to 2). The last hidden layer of the model is therefore of size 128. We were able to reproduce similar results to the original paper~\cite{antipov2017effective}.\\
\emph{\underline{Attrib-CelebA}: detecting 40 binary face attributes.}
Even if applying the same metrics as in~\cite{cao2018partially}, we use a simple PyramidNet-50 and only one linear layer for all 40 attributes, with a Binary Cross Entropy Loss. The error rate is computed with a threshold of 0.5. The last hidden layer of the model is of size 376. We achieve an average error rate of 8.03, which is not on par with state-of-the-art (7.02)~\cite{cao2018partially}.\\
\emph{\underline{Object-ImageNet}: classifying images among ImageNet classes.}
Even if models trained on ImageNet are not designed for face analysis, they were often used in transfer learning because of the quality of the learned features. Therefore, we simply reuse an already trained ResNet-50 achieving 7.13 top-5 error on ImageNet. The last hidden layer of the model is of size 2048.

\paragraph{Tasks for evaluating the knowledge transfer}
To evaluate our transfer learning approach, we carefully designed 10 tasks based on 7 different datasets with diverse sizes, annotations and associated methods (\eg architectures). They are called {\em evaluation datasets} and {\em evaluation tasks} in the rest of the paper. These 10 evaluation tasks are related to the 6 previous tasks (sources of knowledge), but in most cases are not using the same domains nor the same objectives.

\noindent\emph{\underline{Attrib-CelebA}:} We also use this dataset for evaluation. Indeed it allows to have one common dataset used as the source of knowledge and for evaluation tasks. Thus we can quantify the interest of the approach that is proposed to improve already known tasks. By the way the test set of CelebA has never been seen by the pre-trained model.\\ 
\emph{\underline{AgeR-UTK}, \underline{AgeC-UTK}, \underline{Gender-UTK}, \underline{Race-UTK}:} UTKFace~\cite{utk} is a dataset annotated with gender, age and race. We can therefore define such tasks with this dataset. Age classification among 7 age categories (AgeC-UTK), gender prediction (Gender-UTK) and race prediction among 5 classes (Race-UTK) are evaluated with micro recall on the subsets defined in~\cite{das2018mitigating}. Finally, the real age regression (AgeR-UTK) is achieved following the approach described in~\cite{cao2019consistent}, using mean absolute error (MAE).\\
\emph{\underline{AgeR-FG}:} FG-NET~\cite{fgnet} is a dataset of 1002 faces annotated in real-valued age. We follow a leave-one-person-out protocol proposed by~\cite{antipov2017effective} for age regression in MAE.\\
\emph{\underline{Expr-SFEW}:} The task is to predict the facial expression between 7 classes (\eg, 'angry'). SFEW~\cite{sfew} is a small dataset of 1766 images extracted from movies and displaying diverse facial expressions. We follow the same approach as~\cite{vielzeuf2018occam} providing the micro recall on the validation set, as the test set labels are not available.\\
\emph{\underline{Expr-RAF}:} RAF~\cite{raf} is a larger dataset (15339 images) with a reliable annotation of the 7 facial expressions. We also provide a micro recall on the test set as in~\cite{zeng2018facial}.\\
\emph{\underline{Pain-UNBC}:} UNBC-ShoulderPain~\cite{pain} is a video dataset, containing a total of 48391 recorded frames of diverse people faces displaying different levels of pain. Several protocols exist in the literature. We choose to follow the protocol of~\cite{zhang2018bilateral} (but with all frames annotations) and estimate the pain intensity level of a given frame with a number between 0 and 6. We also follow a leave-one-person-out approach and report the MAE.\\
\emph{\underline{Identity-LFW}:} We consider the same task as Identity-MS, but without using any annotated dataset such as MS-Celeb.

\begin{table}[tb]
\centering
\begin{tabular}{lll}
\hline
Dataset      & \# Detected Faces  & \# Undetected Faces \\ \hline
CelebA       & 202442 & 177        \\
UTKFace      & 24018  & 98          \\
FG-NET       & 1002    & 0            \\
SFEW         & 1732   & 37          \\
RAF          & 15330  & 9        \\
ShoulderPain & 48391  & 0            \\
LFW          & 13233  & 0            \\
$\mathcal{D}_{unsup}$ & 4.12 M  & 0.02M          \\ \hline
\end{tabular}
\caption{Number of detected/undetected faces for each dataset.}
\label{detection}
\end{table}

\subsection{Implementation details}
\paragraph{Large face dataset} The $\mathcal{D}_{unsup}$ image set used to train the autoencoder is composed of 4.12 M of faces coming from 3 datasets: the training set used by VGGFace2~\cite{cao2018vggface2} (3.14 M), the Emotionet dataset~\cite{fabian2016emotionet} (0.72 M), and the IMDB-WIKI dataset~\cite{imdbwiki} (0.26 M). All the annotations included with these images (identity for VGGFace2, action units for Emotionet and age, gender, identity for IMDB-WIKI) are discarded. Only the images are used. A supplementary set composed of the VGGFace2 test set and the remaining faces from Emotionet and IMDB-WIKI datasets (350,000 faces) are defined as the test set of $\mathcal{D}_{unsup}$ and used to evaluate the autoencoder. There is no image overlap between the {\em evaluation datasets} and $\mathcal{D}_{unsup}$ . 

\paragraph{Data Preprocessing}
We pre-process both $\mathcal{D}_{unsup}$ and the evaluation datasets. We use a private face detector to first detect and loosely crop the detected faces. If more than one face is detected, we select the closest to the image center. A landmark-based aligner is then applied on the detected faces, which are finally resized to 300x300x3 pixels. 
Table~\ref{detection} reports the number of images where a face was detected for each dataset (first column). When a face is not detected (second column), we will consider during evaluation of our models (a) that the prediction is not correct when addressing classification problems (b) and that the prediction is the average between minimum and maximum values when dealing with regression problems. Note that the rest of the paper is following this rule.

\subsection{Experiments on the fusion operator}

\begin{table}[tb]
\centering
\begin{tabular}{lllll|ll}
\hline
Modality & PCA  & AE            & VAE  & DAE           & MT   & $\mathcal{S}$ \\ \hline
Expr     & 0.28 & \textbf{0.23} & 0.26 & 0.26          & 0.55 & 0.39          \\
Identity & 0.25 & \textbf{0.22} & 0.23 & 0.26          & 1.12 & 0.35          \\
Object   & 0.48 & 0.26          & 0.30  & \textbf{0.25} & 0.67 & 0.44          \\
Age      & 0.23 & \textbf{0.19} & 0.22 & \textbf{0.19} & 0.77 & 0.38          \\
Attrib   & 0.33 & \textbf{0.27} & 0.31 & 0.29          & 0.97 & 0.35          \\
Gender   & 0.25 & \textbf{0.25} & 0.27 & 0.27          & 1.22 & 0.30           \\ \hline
Average  & 0.31 & \textbf{0.24} & 0.27 & 0.25          & 0.92 & 0.37          \\ \hline
\end{tabular}
\caption{rRMSE obtained on $\mathcal{D}_{unsup}$ tests set by considered methods for each task and on average.}
\label{table:recon}
\end{table}

\paragraph{Reconstruction quality}
As described in Section~\ref{methods}, our fusion operator takes as input the concatenation of the 6 embeddings $(h_m)$, one per task, giving a vector of size 5488 in our case. It generates a compact representation $h_e$ which size is fixed to 1024 in all the experiments.

We first evaluate the fusion operator by checking its ability to reconstruct the original $h_m$ features from $h_e$. We report in Table~\ref{table:recon} the relative Root Mean Squared Error (rRMSE) between $h_m$ and $\tilde{h}_m$ for diverse fusion operators. PCA stands for Principal Components Analysis, AE for standard Autoencoder, VAE for Variational Autoencoder and DAE for Denoising Autoencoder. The last two columns will be studied later in the paper. Note that AE, VAE and DAE have the same number of parameters (the encoder $\mathcal{F}$ has 3 fully connected layers: 5488$\times$3136, 3136$\times$1792 and 1792$\times$1024 and the decoder $\tilde{\mathcal{F}}$ is the symmetrical). 
The PCA baseline is easily outperformed by other approaches. The two best performing are the AE and the DAE. Surprisingly, the DAE does not generalize better than the AE, and is performing better only for the reconstruction of the ImageNet modality, which is the less relevant in a context of face inputs. For the rest of the paper, we therefore choose the encoder of the simple AE as our Fusion Operator $\mathcal{F}$.

Nevertheless, a lower rRMSE is not a guarantee of better performance when applying the representation on other tasks and datasets. Thus, we  most of all must evaluate the $h_e$  in transfer learning experiments.

For each evaluation task, we experimented several alternatives summarized  Table~\ref{tab:ae_results}. As a baseline,  we first evaluate a  Multi Layer Perceptron taking as input the concatenation (Concat) of all modalities ($\bigcup\limits_{m=1}^{6} h_m $) and having the architecture of the AE encoder. The model is trained on the training set of the considered task. 
We also compare the benefits brought by two of the previously presented fusion operators, the Princpal Components Analysis (PCA) and the autoencoder (AE). In this case, the $h_e$ representation of size 1024 is first extracted from the training data and then used to train a small Multi Layer Perceptron. 
Finally, another concurrent approach consists in selecting the modality (or embedding) yielding the Best Transfer (BT) or even the Best Combination of modalities Transfer (BCT). The authors of~\cite{zamir2018taskonomy} proposed a method to automatically select such a best combination of features. We choose here to reproduce this approach in a naive way, by brute force testing all the possible single transfers (BT) or combinations (by concatenation) of transfers (BCT) and reporting the best found results.

\begin{table}[tb]
\centering
\begin{tabular}{llllll}
\hline
Dataset       & \multicolumn{3}{c}{Fusion Operators}     & \multicolumn{2}{c}{Selection} \\ \hline
              & Concat & PCA  & AE             & BT        & BCT               \\ \cmidrule(lr){2-4} \cmidrule(lr){5-6}
Attrib-CelebA & 8.07   & 8.03 & \textbf{7.70}   & 8.03      & 7.85              \\
AgeR-UTK      & 4.45   & 4.68 & \textbf{4.39}  & 4.70       & 4.54              \\
AgeC-UTK      & 65.50   & 65.00   & \textbf{68.80}  & 63.2      & 67.20              \\
Gender-UTK    & 96.92  & 96.7 & \textbf{97.20}  & 96.50      & 97.10              \\
AgeR-FG       & 3.22   & 3.18 & \textbf{2.85}  & \textbf{2.85}      & \textbf{2.85}            \\
Expr-SFEW     & 45.70   & 32   & 52.10           & 52.20      & \textbf{53.1}     \\
Expr-RAF      & 84.89  & 81.9 & \textbf{86.51} & 85.48     & 85.74             \\
Pain-UNBC     & 0.69   & 0.6  & 0.54           & 0.53      & \textbf{0.51}     \\
Race-UTK      & 86.65  & 62.5 & \textbf{89.20}  & 83.40      & 86.20              \\
Identity-LFW  & 88.10  & 96.8 & 99.10           & 99.65     & \textbf{99.7}     \\ \hline
\end{tabular}
\caption{Performance of fusion and selection approaches on the 10 evaluation tasks (performance metrics are given in Section~\ref{sec:datasets}).}
\label{tab:ae_results}
\end{table}

\begin{table*}[ht]
\centering
\begin{tabular}{ll|lllll|ll}
\hline
Dataset       & Metric     & CNN     & \multicolumn{2}{c}{MT} & \multicolumn{2}{c}{$S$} & Teacher            & State-of-the-art (\# parameters)                                                       \\ \hline
              &            &         & CF        & WF         & CF     & WF             &               &                                                                                        \\\cmidrule(lr){4-5} \cmidrule(lr){6-7} 
Attrib-CelebA & Error Rate & 8.60    & 8.12      & 8.04       & 7.81   & 7.67           & 7.70           & \textbf{7.02~\cite{cao2018partially}}(16 M)                                            \\
AgeR-UTK      & MAE        & 6.38    & 4.70       & 4.42       & 4.24   & \textbf{4.05}  & 4.39          & 5.39~\cite{cao2019consistent}(21.8 M)                                                  \\
AgeC-UTK      & Recall     & 57.80    & 67.90      & 68.40       & 68.80   & \textbf{70.40}  & 68.80          & 70.10~\cite{das2018mitigating}(5 M)                                                     \\
Gender-UTK    & Recall     & 90.00      & 93.15     & 94.4       & 97.58  & 97.90           & 97.20         & \textbf{98.23~\cite{das2018mitigating}} (5 M)                                          \\
AgeR-FG       & MAE        & 11.10    & 3.95      & 3.12       & 2.95   & 3.05           & \textbf{2.85} & \textbf{2.81-3.00}~\cite{rothe2018deep}~\cite{antipov2017effective} (25 M)              \\
Expr-SFEW     & Recall     & 22.00      & 50.20      & 52.20       & 54.00     & \textbf{57.2}  & 52.10          & \textbf{55.40-58.14~\cite{vielzeuf2018occam}~\cite{acharya2018covariance}} (1.7 M/5 M) \\
Expr-RAF      & Recall     & 69.00      & 82.40      & 87.20       & 87.30  & \textbf{89.3}  & 86.51         & 86.77~\cite{zeng2018facial} (35 M)                                                     \\
Pain-UNBC     & MAE        & 0.89    & 0.64      & 0.72       & 0.56   & 0.52  & 0.54          & \textbf{0.51~\cite{zhang2018bilateral}} (0.0001 M)                                     \\
Race-UTK      & Recall     & 62.20    & 81.20     & 82.20       & 88.2   & \textbf{91.20}  & 89.20          & 90.10~\cite{das2018mitigating} (5 M)                                                    \\
Identity-LFW  & Pairs      & (98.40) & 94.27     & (99.1)     & 98.92  & (99.42)        & 99.10          & \textbf{99.65-99.87}~\cite{schroff2015facenet}(25 M)                                   \\ \hline
\end{tabular}
\caption{Performance of diverse end-to-end methods evaluated on the 10 evaluation tasks (performance metrics are given in Section~\ref{sec:datasets}).}
\label{tab:cnn_results}
\end{table*}
Table~\ref{tab:ae_results} shows that the Concat baseline is outperformed by all other approaches on almost all evaluated tasks. This might be explained by the large dimensionality of the input of the Concat method and the limited size of some of the training sets. Moreover, this is also inline with the fact that the best performing combination of modalities is often not the combination of all modalities.

In addition, it is also interesting to see that the simple PCA method is nevertheless several times on par with the BT results, while the AE performances are better than BT results and often better than the BCT. 
This enlightens the first important finding of this paper. \emph{When the embeddings from which we want to transfer knowledge are correlated, there is a benefit to exploit these redundancies instead of discarding some information by block}. It is in line with what is usually observed in multimodal fusion problems. Even if some modalities do not perform well alone, they can bring crucial complementary information. In contrast to the Concat approach, fusion operators are able to extract meaningful fused representations from the modalities because of the large number of observed samples of $\mathcal{D}_{unsup}$.

\subsection{Experiments on the distillation process}
The Teacher is made of the six models trained separately on different tasks and combined by the fusion operator. It results in a very large number of parameters (127M in total). Thus, it leads to a huge computational burden and makes it difficult to use in real-world applications. Moreover, we can't easily adapt the full model to a new problem.
To tackle these issues, we proposed a subsequent distillation step transferring the knowledge of the 6 models as well as the fusion operator to a single light-weight model. We use a ResNet-18 network as backbone in all these experiments.

In Table~\ref{tab:cnn_results} we compare the proposed distillation process with two alternatives: First,  the so-called 'CNN' approach consists in directly training the backbone network on the evaluation tasks. It stands as the most naive baseline.  Second, the 'Multi-Task approach' (MT) consists in training the backbone network in a multitask fashion on $\mathcal{D}_{unsup}$. To do so we plug a decoder on top of the last hidden layer of the backbone to predict the $(h_m)_{m\in(1..6)}$ associated the input image. This decoder presents the same architecture as the Teacher's AE decoder. Then the transfer is done in the same fashion as in the step 3 of our method. We use the backbone network as an image encoder and plug a MLP\footnote{The MLP is composed of 2 layers (1024 to 512, 512 to output) with batchnorm and elu activation for first layer.} denoted as $\mathcal{C}$ in Figure~\ref{fig:overview} on top of it. In Table~\ref{tab:cnn_results}, we report two scores: the classifier fine-tuning (MT-CF) score, where only $\mathcal{C}$ is optimized; and the whole fine-tuning (MT-WF) score, where we back-propagate the gradient in the whole model.

The distilled Student is also characterized by two scores: the classifier fine-tuning ($\mathcal{S}$-CF) score, where only $\mathcal{C}$ is optimized; and the whole fine-tuning ($\mathcal{S}$-WF) score, where we back propagate the gradient to the entire network. For easier comparison, the Teacher results (which are also in AE in Table~\ref{tab:ae_results}) are provided.

Table~\ref{tab:cnn_results} details the results obtained by all options on the considered tasks.
Note that for the specific case of LFW, two types of results are reported. For Teacher, MT-CF and $\mathcal{S}$-CF, the results are obtained without any fine-tuning, directly using the $h_e$ or $h_S$ representation. For other methods, the result is given between parenthesis. Before evaluation on LFW, the network is first trained (or fine-tuned) on a subset of 100,000 faces from VGGFace2 to predict Identity.

The CNN baseline is outperformed by all other methods, validating the benefits brought by transfer learning.
We then compare the MT and the Student approaches. MT is outperformed on all tasks by $\mathcal{S}$. Moreover MT results are almost always lower than  Teacher's results except for the expression recognition task, where MT-WF outperforms the Teacher on RAF and is on par with the Teacher on SFEW. 

Coming back to Table~\ref{table:recon}, the last two columns report the rRMSE obtained when asynchronously training a decoder to reconstruct the original $h_m$ from the representation obtained by image encoding. The column relative to MT shows that the error is relatively low on Expression, ImageNet and Age but explodes on Identity and Gender. The same behaviour is observed in the Table~\ref{tab:cnn_results}. MT performs especially bad on Identity-related tasks such as Identity, Race or Gender. It empirically underlines a link between the reconstruction error observed on $\mathcal{D}_{unsup}$ and the performance on the evaluation tasks.

Another interesting point is the comparison between the Teacher and the Student.
When the Student is only fine-tuned at classifier-level ($\mathcal{S}$-CF), both models perform equally. These results also show that even if the Student $\mathcal{S}$-CF does not have the same reconstruction ability as the Teacher (see Table~\ref{table:recon}), it achieves similar and sometimes even better results than the Teacher when transferred to novel tasks. This might be explained by the fact that the Student is not able to overfit the $\mathcal{D}_{unsup}$ dataset. Note that $\mathcal{S}$-CF may also benefit from data augmentation, which boosts the performance on RAF for instance.

Then, when the Student is entirely fine-tuned ($\mathcal{S}$-WF), the Teacher is outperformed on almost every tasks, confirming the intuition developed in Section~\ref{methods} about the benefit of a general fine-tuning for better domain adaptation. Moreover, the Student $\mathcal{S}$ is deeper than the AE (fusion operator) and the rest of the Teacher can't be fine-tuned at a reasonable cost. Finally, this is in line with the deep students outperforming their teachers in~\cite{romero2014fitnets}.

In the particular case of FG-NET, the loss of performance coming from the whole fine-tuning might be explained by the small size of the training set and the absence of benefits from data augmentation due to relatively controlled quality of images.

\subsection{Do we improve the original models?}
To answer this question we compare the original models (those used as knowledge sources) to the Teacher and the Student in Table~\ref{tab:origin}, on the original tasks. For Expression, Attributes and Gender we observe a clear improvement, while for the Age the performance is slightly degraded. For the Identity, it is difficult to compare, as we did not fine-tune $\mathcal{S}$ on the same set as the original model. Nevertheless, on the LFW benchmark the Student is outperformed by the original by a gap of 0.23\%. Finally, to avoid a long training time we do not compare the models on ImageNet but on the smaller dataset TinyImageNet~\cite{yao2015tiny}. The obtained accuracy (on the validation set) clearly underlines the importance in the choice of $\mathcal{D}_{unsup}$: the unsupervised training has been done only on face images and thus is not beneficial for tasks such as ImageNet classification. Despite this loss in performance, note that when training our ResNet-18 from scratch on TinyImageNet, we achieve only 52\% accuracy.

\begin{table}[tb]
\centering
\begin{tabular}{llll}
\hline
Dataset & Original & Teacher &  Student             \\ \hline
Expr-AffectNet         & 63.5                         & 64.0                        & \textbf{64.4} \\
Attrib-CelebA         & 8.03                         & 7.7                         & \textbf{7.67} \\
Gender-UTK            & 96.5                         & 97.2                        & \textbf{97.9} \\
AgeR-FG               & \textbf{2.85 }                        & \textbf{2.85}                        & 3.05          \\
Identity-LFW              & \textbf{99.65}               & 99.1                        & 99.42         \\
Object-TinyImageNet                    & \textbf{76.2}                & 71.8                        & 56.5          \\ \hline
\end{tabular}
\caption{Performance of the original models, of the Teacher and of the Student on the original tasks.}
\label{tab:origin}
\end{table}

\subsection{Number of parameters and Training times}
The number of parameters of our model is an important element. Indeed, it may first explain some differences of performance between the Student and the MT approach.
Indeed the Image encoder $\mathcal{E}_S$ is composed of 1.7M parameters, while the Teacher encoder is composed of 127M parameters (with 103M already trained on other large datasets and frozen in all experiments). The decoders (in AE and MT) have the same architecture with 24.6M parameters. 

Therefore both the capacity and the number of seen examples of the Teacher encoder may help to solve the difficult task of compression and reconstruction of the diverse modalities. Moreover the MT architecture is unbalanced, in the sense that the decoder is more than 13.5 times bigger than its encoder, which might complicate the training.

Another important observation is the comparison between the Teacher and the Student. The number of parameters has been reduced by a factor of 75 without loss of performance in terms of transfer learning. It both shows that a deep fine-tuning brings benefits over simple representation transfer and that a lower number of parameters can lead to better generalization ability. Indeed, when compared to state-of-the-art models (see last column of Table~\ref{tab:cnn_results}), the Student with its 2.2M parameters (1.7M for encoder $\mathcal{E}_S$ and around 0.5M for $\mathcal{C}$) is often smaller than its competitors.

Finally, we report from Figure~\ref{fig:times} the training time spent on $\mathcal{D}_{unsup}$ and on the evaluation datasets for all the methods. Even if the training on $\mathcal{D}_{unsup}$ is relatively long (70 hours), the transfer learning step is then really faster than training a model from scratch. Moreover compared to the brute-force baseline of selecting all possible combinations (BCT), the training time of the Student is divided by 4.
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/time.pdf}
    \caption{Training time in hours (logscale) for all methods on $\mathcal{D}_{unsup}$ when relevant (Encode) and on the evaluation datasets (Transfer). Extract is the feature extraction step for all $E_m$}
    \label{fig:times}
\end{figure}






==> methods.tex <==
\section{Methodology}
\label{methods}
\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/2203_overview.pdf}
    \caption{Overview of the method. Step 1 shows the Teacher model, learning to encode images into a compact join embedding. It is composed of a feature extraction part $(E_m)_{m\in (1..M)}$, followed by a fusion operator $\mathcal{F}$ trained to minimize the loss $\mathcal{L}_{Fusion}$. Step 2 shows the Student model $\mathcal{S}$. The image encoding part is composed of a convolutional neural network $\mathcal{E}_S$ trained to minimize $\mathcal{L}_{Distillation}$, the distance to the $h_e$ representation of the Teacher. Step 3 consists in transferring on an annotated evaluation dataset. A "classifier" $\mathcal{C}$ is plugged on top of the image encoding module (it may be the Teacher or the Student) and trained to optimize the loss $\mathcal{L}_{Task}$. If the image encoder is the Teacher, only $\mathcal{C}$ $\mathcal{L}_{Task}$ is trained to fit, whereas in the case of $\mathcal{E}_S$ as image encoder, the back-propagation is done both in $\mathcal{C}$ and $\mathcal{E}_S$.}
    \label{fig:overview}
\end{figure*}

As stated in the introduction, we assume having $M$ existing models denoted as $E_m$ where $m$ is the $m^{th}$ model. Each model provides an embedding  from the image space to a feature space $h_m$ in which the inference is done. Our goal is to produce a general embedding, called $h_e$, common to all the existing tasks and usable for novel tasks for which we only have a few training images.

We address this problem in a three-step approach (see Fig.~\ref{fig:overview}). 
First, we define a common embedding by aggregating existing models through a fusion operator (denoted as $\mathcal{F}$).
%which is the key contribution of the paper. 
We explored different fusion operators but basically, it consists in aggregating the features given by the various models into a single vector, by learning an autoencoder with such features, on a large dataset. The common embedding $h_e$ is the hidden layer of the autoencoder.

Second, we introduce a Teacher/Student distillation step to learn a compact Student model ($\mathcal{S}$) doing the same mapping as the whole collection of fused models. In other words, $\mathcal{S}$   directly provides $h_e$ from an input sample $x$.

Third, the compact student model $\mathcal{S}$ is entirely fine-tuned on novel tasks.

\subsection{Computing the Teacher Model}
The aim of the Teacher Model is to benefit from the knowledge embedded in the existing models for learning a mapping from the input data into a common compact space, regardless of the number of parameters. %As shown in Figure~\ref{fig:overview} the Teacher is divided into two parts: i) image encoding, ii) knowledge transfer.

We assume having a large unlabeled dataset denoted as $\mathcal{D}_{unsup}$. Each image of this dataset can be encoded by the M features extractors available, denoted as $(E_m)_{m\in (1..M)}$. These M features extractors may come from existing models trained on diverse domains and tasks or may be hand-crafted features extractors. In our case, each feature extractor takes an image $x\in \mathcal{D}_{unsup}$ as input and outputs an embedding $h_m$. These M different embeddings $(h_m)_{m\in(1..M)}$ may be seen as different views or modalities of the same data.
Each $h_m$ is individually rescaled between -1 and 1 to ensure homogeneity. 
 
Let now $\mathcal{F}$ be a multimodal fusion operator defined by:
\begin{equation}
    h_e = \mathcal{F} ((h_m)_{m\in(1..M)})
\end{equation}
where $h_e$ is a compact embedding containing information from all the previously obtained embeddings.

A naive definition of $\mathcal{F}$ could be the Identity function, meaning that $ h_e = \bigcup\limits_{m=1}^{M} h_m $. 
However, as they $h_m $ may include redundancy, cross-correlation and may be noisy views of the input image, there is a huge interest in finding a more compact and robust representation. 

We propose to build the fusion operator as the encoder part of an autoencoder, learned on the features computed from the samples of $\mathcal{D}_{unsup}$ .
If the output of the decoder part $\tilde{\mathcal{F}}$ is denoted as $(\tilde{h}_m)_{m\in(1..M)} = \tilde{\mathcal{F}}(h_e)$,
the loss of the autoencoder can be defined by:
\begin{equation}
    \mathcal{L}_{Fusion} = \Sigma_{m=1}^M || \tilde{h}_m - h_m ||^2
\end{equation}

We discuss the exact architecture of the autoencoder in the experiments section. We experimented with PCA, regular autoencoders~\cite{ballard1987modular}, variational autoencoders~\cite{kingma2013auto} and denoising autoencoders~\cite{vincent2010stacked}. 

The dimensionality of $h_e$ plays an important role in the fusion step and may be chosen by cross validation. However, as a rule of thumb we fixed it in the experiments as the average dimensionality of the embeddings of the existing models. 


Once the encoder is learned, it can be used as it is by adding a Multi Layer Perceptron (named $\mathcal{C}$ in Figure~\ref{fig:overview}) on top of the $h_e$ representation. In this case, the transfer learning consists in optimizing the parameters of this MLP on a novel target dataset, using the corresponding loss $\mathcal{L}_{Task}$.

\subsection{Computing the Student Model}
The Teacher has a huge number of parameters contained in the different aggregated models $(E_m)_{m\in (1..M)}$ and $\mathcal{F}$, making it impractical for subsequent usages. In this section, we make it  lighter through a distillation process~\cite{HintonVD15}. 


The encoder of the Student model is named $\mathcal{E}_S$ and maps images $x$ into features $h_S$ of the same size as $h_e$. We arbitrarily choose a ResNet~\cite{he2016deep} architecture for the Student as it is known for its good performance on face analysis tasks.

We use the fusion operator $\mathcal{F}$ to supervise the ResNet backbone $\mathcal{E}_S$. Therefore, we keep the fusion operator fixed and train $\mathcal{E}_S$ as:
\begin{equation}
   \underset{\theta_S}{argmin}\  \mathcal{L}_{Distillation}(\theta_S)
\end{equation}
where $\mathcal{L}_{Distillation} = D_c(h_e , h_S)$ for images in $\mathcal{D}_{unsup}$, $\theta_S$ are $\mathcal{E}_S$ parameters and $D_c$ the cosine metric.

It would have been possible to train $\mathcal{E}_S$ and the fusion operator simultaneously, by fitting the features given by the different models $(h_m)_{m\in(1..M)}$, on the samples of $\mathcal{D}_{unsup}$. In this case, there are more parameters to be trained at the same time. We experimentally observed that using the encoder and keeping it fixed make the performance better. 

\subsection{Fine-tuning the student on a novel task}
Once the image encoding $\mathcal{E}_S$ has been successfully learned on $\mathcal{D}_{unsup}$, the transfer learning on the evaluation datasets is straightforward.
As done for the Teacher, a first way to transfer is to extract $h_S$ from the input image and then to train an MLP ($\mathcal{C}$ in Figure~\ref{fig:overview}) on top of it, using an appropriated loss $\mathcal{L}_{Task}$. As $h_S$ is a noisy estimation of $h_e$, the performance can be lower than the Teacher's.
Nevertheless, previous works~\cite{chu2016best} showed that fine-tuning all the parameters of a model may lead to a better domain adaptation and therefore improve the quality of the transfer. Due to the limited capacity of the Student compared to the Teacher's, we fine-tune the whole Student, adapting $\mathcal{E}_S$ to the target dataset.

Moreover, another important benefit of the Student is its similarity to other models used on image datasets, allowing to easily use datasets specific methods such as augmentation or regularization.

